NPC: Neural Point Characters from Video

High-fidelity human 3D models can now be learned directly from videos, typically by combining a template-based surface model with neural representations. However, obtaining a template surface requires expensive multi-view capture systems, laser scans, or strictly controlled conditions. Previous methods avoid using a template but rely on a costly or ill-posed mapping from observation to canonical space. We propose a hybrid point-based representation for reconstructing animatable characters that does not require an explicit surface model, while being generalizable to novel poses. For a given video, our method automatically produces an explicit set of 3D points representing approximate canonical geometry, and learns an articulated deformation model that produces pose-dependent point transformations. The points serve both as a scaffold for high-frequency neural features and an anchor for efficiently mapping between observation and canonical space. We demonstrate on established benchmarks that our representation overcomes limitations of prior work operating in either canonical or in observation space. Moreover, our automatic point extraction approach enables learning models of human and animal characters alike, matching the performance of the methods using rigged surface templates despite being more general. Project website: https://lemonatsu.github.io/npc/

==> figures/exps/fig_ablation.tex <==
\newlength\hmablatscale
\setlength\hmablatscale{0.33\linewidth}
\ifblurface%
\newcommand{\hmablatpost}{_blur}
\else%
\newcommand{\hmablatpost}{}
\fi%
\newcommand{\hmablatpath}{statics/figs/exp/ablation/}
\newcommand{\hmablatma}{No $f^d$}
\newcommand{\hmablatmb}{No $f^\theta$}
\newcommand{\hmablatmc}{No $f^p$}
\newcommand{\hmablatmd}{No $\Delta p$}
\newcommand{\hmablatme}{Ours-full}
\newcommand{\hmablata}{S9_Ours-no-coord_00_np}
\newcommand{\hmablatb}{S9_Ours-no-pose-feat_00_np}
\newcommand{\hmablatc}{S9_Ours-no-point-feat_00_np}
\newcommand{\hmablatd}{S9_Ours-lbs-only_00_np}
\newcommand{\hmablate}{S9_Ours-full_00_np}

\begin{figure}[h]
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\parbox[t]{\hmablatscale}{%
\centering%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath S9_GT_00_np\hmablatpost}%
}\\%
{ Reference image}\\%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath\hmablatc\hmablatpost}%
}\\%
{ \hmablatmc}%
}%
\hfill%
\parbox[t]{\hmablatscale}{%
\centering%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath\hmablata\hmablatpost}%
}\\%
{ \hmablatma}\\%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath\hmablatd\hmablatpost}%
}\\%
{ \hmablatmd}%
}%
\hfill%
\parbox[t]{\hmablatscale}{%
\centering%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath\hmablatb\hmablatpost}%
}\\%
{ \hmablatmb}\\%
\fbox{\includegraphics%
[width=\hmablatscale,trim=80 0 0 0,clip]%
{\hmablatpath\hmablate\hmablatpost}%
}\\%
{ \hmablatme}%
}%
\centering%
\caption{\textbf{Ablation study on unseen poses.} Our proposed features $f^d$, $f^\theta$ and $f^p$  enables \ourapproach{} to achieve better overall perceptual quality, with less noises and improved consistency on the texture.
}%
\label{fig:exp-ablation}
\end{figure}

==> tables/table_supp_NN_search.tex <==
\begin{table}[t]
\caption{\textbf{Tabulated K-NN overlaps with the naive K-NN with high probability}. We report the neighbor overlap rate between ours and the naive K-NN for $k=8$  , as well as the coverage rate of the $k$-th naive nearest neighbors.}
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cccccc}
\toprule
1st & 2nd & 3rd & 4th & 5th & Overlap rate (all eight)\\
\midrule%
\rowcolor{Gray}
100\% & 86.4\% & 81.5\% & 75.9\% & 69.9\% & 72.6\% 
\end{tabular}
\label{tab:supp-nn-search}
}
\end{table}

==> tables/table_supp_SMPL_init.tex <==
\begin{table}[t]
\caption{\ourapproach{} can also use SMPL~\cite{loper2015smpl} surface points for initialization.}
\centering
\resizebox{0.8\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
 & PSNR~$\uparrow$  & LPIPS~$\downarrow$  \\
\midrule
 \rowcolor{Gray}
DANBO init. & 24.86 (+0.00\%) & 0.115 (+0.00\%) \\
SMPL init. & 24.90 ({\color{green}+0.02\%})&  0.116 ({\color{red}+0.90\%}) \\
\end{tabular}
\label{tab:supp-smpl-init}
}
\end{table}

==> tables/table_supp_full_ablation.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on each of our proposed designs.} Most of our features contribute to the final perceptual quality.}
\centering
\resizebox{0.75\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}
\toprule
 & KIDx100~$\downarrow$  & LPIPS (VGG)~$\downarrow$ & LPIPS (Alex)~$\downarrow$ \\
\midrule
No $f^d$ & 5.54& 0.122 & 0.132\\
\rowcolor{Gray}
No $f^p$& 4.51& 0.122 & 0.131\\
No $f^\theta$& 4.50& 0.120 & 0.132\\
\rowcolor{Gray}
No $\Delta p$& 4.61& 0.120 & 0.131\\
No $f^v$ & 4.48&  0.115 & \textbf{0.124}\\
\rowcolor{Gray}
No $r_i$& \textbf{3.87}& 0.116 &  0.125\\
\midrule%
\textbf{Ours full}& 4.43 & \textbf{0.115} & \textbf{0.124}\\
\end{tabular}
\label{tab:supp-ablation}
}
\end{table}
